The Price of Differential Privacy under Continual Observation

We study the accuracy of differentially private mechanisms in the continual release model. A continual release mechanism receives a sensitive dataset as a stream of $T$ inputs and produces, after receiving each input, an accurate output on the obtained inputs. In contrast, a batch algorithm receives the data as one batch and produces a single output. We provide the first strong lower bounds on the error of continual release mechanisms. In particular, for two fundamental problems that are widely studied and used in the batch model, we show that the worst case error of every continual release algorithm is $\tilde \Omega(T^{1/3})$ times larger than that of the best batch algorithm. Previous work shows only a polylogarithimic (in $T$) gap between the worst case error achievable in these two models; further, for many problems, including the summation of binary attributes, the polylogarithmic gap is tight (Dwork et al., 2010; Chan et al., 2010). Our results show that problems closely related to summation -- specifically, those that require selecting the largest of a set of sums -- are fundamentally harder in the continual release model than in the batch model. Our lower bounds assume only that privacy holds for streams fixed in advance (the "nonadaptive" setting). However, we provide matching upper bounds that hold in a model where privacy is required even for adaptively selected streams. This model may be of independent interest.

==> continual-release submissionJan6/macros.tex <==
% \parindent=0pt % disables indentation
% \parskip = 1em % sets spacing between paragraphs

\def\podsmac{1}


\usepackage[utf8]{inputenc}
\usepackage{bbm}

\ifnum\pods=0
\usepackage{amssymb} %%for conference format
\else
\fi

\ifnum\pods=0
\usepackage[dvipsnames]{xcolor} %%for conference format
\else
\fi


\usepackage{amsmath,fullpage}
\usepackage{amsthm}
%\usepackage[framemethod=TikZ]{mdframed}
\usepackage{physics}
\usepackage{algorithm,algorithmicx}
\usepackage{subfiles} 
\usepackage[noend]{algpseudocode}
\usepackage{comment}
\usepackage{xspace}
\usepackage[inline,shortlabels]{enumitem}
\usepackage{mathtools}
\usepackage{ulem} \normalem

\usepackage{setspace}
\usepackage{hyperref}
\usepackage{cleveref}


\let\oldemptyset\emptyset
\let\emptyset\varnothing

%%%%%%%%% Environments %%%%%%%%%%
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{remark}{Remark}

\newenvironment{note}
    {\textsc{Note:}}
    {}
  
%%%%%%%%% Font %%%%%%%%%%%
\newcommand{\msf}{\mathsf} %mathsf


%%%%%% For Algorithmic %%%%%%%%%%
\newcommand{\multiline}[1]{%
  \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    #1
  \end{tabularx}
}

\usepackage{stackengine}
\setstackEOL{\\}

\algnewcommand{\LineComment}[1]{\Statex \(\triangleright\) \begin{small}{\emph #1}\end{small} }



%%%%%%%%% DP Symbols %%%%%%%%%%%%
\newcommand{\CR}{nonadaptive continual release model} %non-adaptive continual release 
\newcommand{\aCR}{adaptive continual release model} % adaptive continual release
\renewcommand{\epsilon}{\varepsilon} %epsilon
\newcommand{\eps}{\varepsilon} %epsilon
\newcommand{\X}{\mathcal{X}} %input distribution
\newcommand{\Z}{\mathcal{Z}} %output distribution
\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\left(#1\right)}} %asymptotic O
\newcommand{\dset}{y} %dataset entry
\newcommand{\dstream}{x} %data stream entry
\renewcommand{\vec}[1]{{\bf #1}} %for full (dataset/datastream)
\newcommand{\dstreamvec}{\vec{x}}
\newcommand{\avec}{\vec{a}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\random}{ } %random (dataset/datastream)
\newcommand{\xt}{\vec{\dstream}_{[t]}} %records 1 through t
\newcommand{\node}{v}
\newcommand{\nodeval}{s}
\newcommand{\adv}{\ensuremath{\mathcal{A}\mathit{dv}}\xspace} %adversary
\newcommand{\process}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\mech}{\ensuremath{\mathcal{M}}\xspace} %mechanism
\newcommand{\alg}{\ensuremath{\mathcal{A}}\xspace} %algorithm
\newcommand{\privgame}{\ensuremath{\mathcal{G}}\xspace} %privacy game
\newcommand{\Sim}{\mathcal{S}\text{im}} %Simulator
\newcommand{\DP}[1]{$\mathrm{DP}_{\mathrm{#1}}$} %DP sub
\newcommand{\maxsum}[1]{\ensuremath{\mathrm{\sf MaxSum}_{#1}}} %maxsum problem
\newcommand{\topkselection}{\ensuremath{\mathrm{Top}\text{-$k$ }\mathrm{Selection}}} %top-k-selection problem
\newcommand{\kindselection}[1]{\ensuremath{\text{$k$-}\mathrm{\sf Select}_{#1}}} %top-k-selection problem
\newcommand{\marginals}[1]{\ensuremath{\mathrm{\sf Marginals}_{#1}}} %marginals
\newcommand{\selection}[1]{\ensuremath{\mathrm{\sf SumSelect}_{#1}}} %selection problem
\newcommand{\idealgauss}{\mech_{\msf{gauss}}}
\newcommand{\idealrecomp}{\mech_{\msf{comp}}}
\newcommand{\err}{\text{\sf ERR}} %err
\newcommand{\view}{\mathcal{V}} %view of adversary in the adaptive game
\newcommand{\topkcoord}[1]{#1_{\sf{topk}}} %topk-coordinates
\newcommand{\side}{\text{\sf side}} %side
\newcommand{\gauss}{\ensuremath{\mathcal{N}}} %gaussian distribution
\newcommand{\Gauss}{\gauss} % gaussian distribution
\newcommand{\Lap}{\mathsf{Lap}}

%%%%%%%%%%%%%% random %%%%%%%%%%%%%%%%%%
\newcommand{\messyval}{m}

%%%%%%%%%% General Symbols %%%%%%%%%%
\newcommand{\lra}{\longrightarrow} %long right arrow
\newcommand{\zo}{\{0,1\}} %binary strings
\newcommand{\oneo}{\{-1,1\}} %binary strings
\newcommand{\xor}{\oplus} %xor
\newcommand{\Q}{\mathbb{Q}} %rationals
\newcommand{\R}{\mathbb{R}} %reals
\newcommand{\N}{\mathbb{N}} %naturals
\newcommand{\bigO}{\BigO}
\newcommand{\polylog}{\mathrm{polylog}} %polylog
\newcommand{\defeq}{\overset{\text{\tiny def}}{=}} %defeq
\DeclareMathOperator*{\E}{\mathbb{E}} % expectation
\DeclareMathOperator*{\argmax}{arg\,max} %argmax
\DeclareMathOperator*{\argmin}{arg\,min} %argmin
\newcommand{\setrandomly}{\ensuremath{\xleftarrow{\$}}} % picking randomly from a distribution
\newcommand{\expectederr}[2]{\err_{#1,#2}} %expected error of mechanism


\newcommand{\set}[1]{{\left \{  {#1} \right\} }}
\newcommand{\bit}[1]{{\{0,1\}^{#1}}}

\newcommand{\paren}[1]{{\left ( {#1} \right)}}
\newcommand{\bparen}[1]{{\big ( {#1} \big)}}
\newcommand{\Bparen}[1]{{\Big ( {#1} \Big)}}



%%%%%%%%%%%%%% Comments %%%%%%%%%%%%%
\newcommand{\sat}{\textcolor{red}}
\newcommand{\foradam}{\textcolor{gray}}
\definecolor{mygreen}{rgb}{0.0, 0.49, 0.28}


\ifnum\notes=1 %%% Preliminary version with notes
\newcommand{\srnote}[1]{{\color{blue}\footnote{{\color{blue} {\bf SR:} #1}}}}
\newcommand{\pjnote}[1]{{\color{mygreen}\footnote{{\color{mygreen} {\bf P:} #1}}}}
\newcommand{\ssnote}[1]{{\color{red}\footnote{{\color{red} {\bf SS:} #1}}}}
\newcommand{\asnote}[1]{{\color{brown}\footnote{{\color{brown} {\bf A:} #1}}}}
\newcommand{\old}[1]{\sout{#1}}
\else
\newcommand{\srnote}[1]{}
\newcommand{\ssnote}[1]{}
\newcommand{\pjnote}[1]{}
\newcommand{\asnote}[1]{}
\newcommand{\old}[1]{}
\fi 

\ifnum\notes=1
\newcommand{\sr}[1]{{\color{blue} #1}}
\newcommand{\pj}[1]{{\color{mygreen} #1}}
\newcommand{\sstext}[1]{{\color{red} #1}}
\newcommand{\as}[1]{{\color{brown} #1}}
\else % notes just appear black
\newcommand{\sr}[1]{#1}
\newcommand{\pj}[1]{{#1}}
\newcommand{\sstext}[1]{{#1}}
\newcommand{\as}[1]{{#1}}
\fi


==> continual-release submissionJan6/upperbound-table.tex <==
\ifnum\pods=1
\begin{table*}[t]
\begin{tabular}{|c||c|c|c|c|}
\hline  
   & \multicolumn{2}{c|}{$\rho$-zCDP}  & \multicolumn{2}{c|}{$(\eps,0)$-DP}  \\
   \cline{2-5}
     Problem      & Tree & Recomputation & Tree  & Recomputation  \\
     \hline \hline 
     \maxsum{} 
     & \( \frac{\sqrt{d} \log T \sqrt{\log(dT)}}{\sqrt{\rho}} \)
     & \( \sqrt[3]{\frac{T\log T}{\rho}} \)
     & \( \frac{d (\log d) \log^3 T}{\eps} \)
     & \(\sqrt{\frac{T\log T}{\eps}} \)
     \\
     \hline 
     \selection{} 
     & \( \frac{\sqrt{d} \log T \sqrt{\log(dT)}}{\sqrt{\rho}} \)
     & \( \frac{T^{1/3}\log^{2/3}(d T)  }{\rho^{1/3}} \)
     & \(  \frac{d (\log d) \log^3 T}{\eps} \)
     & \(\sqrt{\frac{T\log (dT)}{\eps}} \)
     \\
     \hline 
\end{tabular}
\caption{Our (asymptotic) upper bounds on the error of DP mechanisms in the adaptive continual release model.}    
\label{tab:algorithmic-results}
\end{table*}
\else
\fi
% \begin{table}[t]
% \begin{tabular}{|c||c|c|c|}
% \hline 
% & & \maxsum{} & \selection{}\\
% \hline \hline 
%  & Tree &  \( \frac{\sqrt{d} \log T \sqrt{\log(dT)}}{\sqrt{\rho}} \) & \( \frac{\sqrt{d} \log T \sqrt{\log(dT)}}{\sqrt{\rho}} \)\\
% \cline{2-4}
% {$\rho$-zCDP} & Recomputation & \(\frac{T^{1/3} \sqrt{\log T}}{\rho^{1/3}} \) & \( \frac{T^{1/3}\log^{2/3}(d T)  }{\rho^{1/3}} \)  \\
% \hline 
% & Tree & \( \frac{d (\log d) \log^3 T}{\eps} \) & \( \frac{d (\log d) \log^3 T}{\eps} \) \\
% \cline{2-4}
% {$(\eps,0)$-DP} & Recomputation & \(\sqrt{\frac{T\log T}{\eps}} \) & \(\sqrt{\frac{T\log (dT)}{\eps}} \)\\
% \hline 
% \end{tabular}
%\caption{Our (asymptotic) upper bounds on the error of DP mechanisms in the adaptive continual release model.}    
%\label{tab:algorithmic-results}
% \end{table}

==> continual-release submissionJan6/upperbounds.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                      UPPER BOUNDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Adaptive Upper Bounds}\label{sec:upper-bounds}
In this section, we define the adaptive continual release model and describe differentially private mechanisms for two types of problems in this model: $\selection{d}$ and approximating functions with bounded sensitivity ($\ell_2$ sensitivity in the case of approximate differential privacy and $\ell_1$ sensitivity in the case of pure DP).  
% $f$ with inputs from ${\zo^*}$ that have $\ell_2$ sensitivity $\Delta_f = 1$ \sstext{(in the case of approximate DP; we require $\ell_1$ sensitivity $\Delta_f = 1$ in the case of pure DP)}. 
Our mechanisms are $(\alpha,T)$-accurate, where the upper bounds for $\alpha$ match the lower bounds obtained in previous sections in the \CR{} up to logarithmic factors in the time horizon $T$, the number of coordinates $d$, and the inverse of the privacy parameter $\frac{1}{\delta}$.

\input{upperbound-table}

%%%%%%%%%%%%%%%%%%% ADAPTIVE MODEL DEFINITION %%%%%%%%%%%%%%%%

\subsection{Adaptive Continual Release}
\label{sec:defs-adaptive}
%https://arxiv.org/abs/2003.14265
%https://arxiv.org/abs/2004.05975
%https://arxiv.org/abs/2101.10836
%Defining privacy for the \aCR{} is more complex than for its nonadaptive variant. 

In the \aCR{}, the input stream given to a mechanism $\mech$ is chosen adversarially. That is, $\mech$ interacts with a randomized adversarial process $\adv$ that runs for $T$ timesteps; at timestep $t \in [T]$, the process $\adv$ receives $a_t$ from $\mech$, updates its internal state, and produces input record $\random{\dstream}_{t+1}$ that is sent to $\mech$ at timestep $t+1$. Process $\adv$ can choose $\dstream_{t+1}$ based on the previous input records $\xt$ and $\mech$'s previous outputs $\vec{a}_{[t]}$. We make no assumptions on $\adv$ regarding running time or complexity; its only limitation is that it does not see the internal coins of $\mech$.

\begin{definition}
A mechanism $\mech$ is  \emph{($\alpha$,T)-accurate} for a function $f$ in the \aCR{} if for all processes $\adv$, the error of $\mech$ with respect to $\adv$ is at most $\alpha$ with high probability, that is,
$$\Pr_{\text{coins of } \mech,\adv} \left[\max_{t\in [T]} \err_f(a_t; \xt) \leq \alpha\right] \geq \frac{2}{3}.$$
\end{definition}

A similar notion of accuracy was considered in work on adversarial streaming \cite{EliezerJWY20, HassidimKMMS20, KaplanMNS21}, though those articles do not directly address privacy.

Next, we define \emph{(event-level) privacy in the \aCR{}} \ifnum\pods=0
, which is trickier than in the \CR{}
\else
\fi
. This concept is implicit in \cite{SmithT13}, but to our knowledge has not been previously defined. Privacy is defined with respect to the game $\Pi_{\mech,\adv}$, described in \Cref{alg:privacy_game}, between mechanism $\mech$ and an adversary $\adv$. In all timesteps except one, $\adv$ outputs a single input record which $\Pi_{\mech,\adv}$ simply forwards to $\mech$. However, there is a special {\em challenge timestep} $t^* \in [T]$, selected by $\adv$, in which $\adv$  provides two records $x_{t^*}^{(L)}$ and $x_{t^*}^{(R)}$. 
The game comes in two versions, specified by its input parameter $\side \in \{L,R\}$ which is not known to $\adv$ or $\mech$: in one version, the record $x_{t^*}^{(L)}$ is handed to $\mech$ at timestep $t^*$; in the other, the record $x_{t^*}^{(R)}$ is handed to $\mech$ instead. The mechanism is private if the distributions on the adversary's view, which consists of its internal randomness and the transcript of messages it sends and receives, 
are close in the two versions of the game.

When the adversary decides in advance on all $T+1$ records that it outputs over the course of the game, the resulting definition is equivalent to the nonadaptive version (Definition~\ref{def:na-privacy}). The version we give here captures a richer class of settings. 

Intuitively, we may think of $x_{t^*}^{(L)}$ as the data of person $t^*$, and of $x_{t^*}^{(R)}$ as a dummy value (say, all 0's). The parameter $\side$ then controls whether the data of person $t^*$ is included in the computation or not. The privacy requirement is that an outside attacker cannot tell whether $t^*$'s data was used, even if the attacker has full knowledge of the process generating the data stream. The adversary $\adv$ combines the data generation process and the attack itself in one entity, so that our model allows for an arbitrary relationship between them.

\newcommand{\rdtype}{\text{\sf type}}
\newcommand{\chall}{\text{\sf challenge}}
\newcommand{\reg}{\text{\sf regular}}

\begin{algorithm}[ht]
\caption{Privacy game $\Pi_{\mech,\adv}$ 
\ifnum\pods=0
for the \aCR{}
\fi
}
\label{alg:privacy_game}
    \begin{algorithmic}[1]
        \Statex \textbf{Input:}  time horizon $T \in \N$, $\side \in \{L, R\}$ (not known to $\adv$).
        \For{\text{$t=1$ to $T$}}
        \State $\adv$ outputs $\rdtype_t \in \{\chall, \reg\}$, where $\chall$ is chosen once during the game.
        % $\adv$ decides if $t$ is the challenge timestep.
            \If{$\rdtype_t = \reg$}
                \State $\adv$ outputs $x_t \in \X$ which is sent to $\mech$.
            \EndIf
            \If{$\rdtype_t = \chall$}
                \State $t^* \gets t$. 
                \State $\adv$ outputs $(x_t^{(L)},x_t^{(R)}) \in \X^2$.
                \State $x_t^{(\side)}$ is sent to $\mech$.  
            \EndIf
            \State $\mech$ outputs $a_t$ which is given to $\adv$.
        \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{definition}
The \emph{view of $\adv$} in privacy game $\Pi_{\mech,\adv}$  consists of $\adv$'s internal randomness and the transcript of messages it sends and receives. Let \emph{$V_{\mech,\adv}^{(\side)}$} denote $\adv$'s  view  at the end of the game run with input $\side \in \{L,R\}$.
% Let \emph{$V_{\mech,\adv}^{(\side)}$} denote \emph{$\adv$'s view} in privacy game $\Pi_{\mech,\adv}$ when it is run with input $\side \in \{L,R\}$. This view consists of $\adv$'s internal randomness and the transcript of messages it sends and receives. 
%its interaction with $\mech$ 
%in privacy game $\Pi_{\mech,\adv}$.
\end{definition}

One could also define the adversary's view as its internal state at the end of the game. The version we define contains enough information to compute that internal state, but is simpler to work with. 
% Note  that this definition of view requires privacy to apply for all possible internal coins of the adversary\srnote{What does it mean that the privacy applies for all possible internal coins of the adversary? First, privacy in the adaptive model has not been defined yet. Second, it is defined as closeness of random variables.}. 

%\ssnote{zCDP undefined, so rho closeness in definition below is undefined without the text I've suggested.} 
In addition to $(\eps,\delta)$-DP, we consider a related notion, called zCDP \cite{BunS16}. See Appendix~\ref{sec:zCDP} for background on zCDP and the notion of $\rho$-closeness of random variables ($\simeq_{\rho})$.

\begin{definition}
A mechanism $\mech$ is \emph{$(\epsilon,\delta)$-DP in the \aCR{}} if, for all adversaries~$\adv$, 
$$V_{\mech,\adv}^{(L)} \approx_{\eps,\delta} V_{\mech,\adv}^{(R)}. $$

\noindent A mechanism $\mech$ is \emph{$\rho$-zCDP in the \aCR{}} if for all adversaries~$\adv$,
\begin{equation*} 
V_{\mech,\adv}^{(L)}\simeq_{\rho} V_{\mech,\adv}^{(R)}. 
\end{equation*}
\sstext{The symbol $\simeq_{\rho}$ denotes $\rho$-closeness (\Cref{def:rho-indistinguishable})}.
\end{definition}


%%%%%%%%%%%%%%%%%%%%% THEOREM STATEMENTS %%%%%%%%%%%%%%%%%%%

\ifnum\pods=1
\subsection{Summary of Adaptive Upper Bounds}\label{sec:adaptive-up-summary}
Our upper bounds on the error of differentially private algorithms for $\maxsum{d}$ and $\selection{d}$ in the adaptive continual release model are summarized in Table~\ref{tab:algorithmic-results}. The corresponding theorems are stated in Section~\ref{sec:adaptive-up-statments}. The upper bounds in the table are attained by two simple mechanisms: one uses the binary tree mechanism and the other recomputes the target function at regular intervals. The bounds stated for $\maxsum{d}$ and obtained via recomputing periodically apply more generally: to all sensitivity-1 functions.


Unlike the proofs of privacy in previous work, the privacy proofs for our adaptive upper bounds (in \Cref{sec:details_ub}) use a simulator that constructs inputs to an underlying mechanism online,  instead of considering only neighboring datasets defined ahead of time.
This allows us to reason about input streams that look very different in different executions of the game (for example, streams whose long-term behavior depends on the mechanism's response at the challenge timestep). 
The accuracy analyses need to account for adaptivity as well.



\else
\fi
%In this subsection, we state theorems that summarize the performance guarantees of our algorithms . 

\ifnum \pods=1
\addcontentsline{toc}{section}{References}
\bibliographystyle{plain}
\bibliography{bibliography}
\appendix
\else
\fi

\ifnum\pods=0
\subsection{Statements of Adaptive Upper Bounds}\label{sec:adaptive-up-statments}
\else
\section{Additional Preliminaries}\label{app:preliminaries}

\subsection{Facts on Differential Privacy}
Differential privacy protects groups of individuals.

\begin{lemma}[Group Privacy~\cite{dwork2006calibrating}]\label{lem:group_privacy} Every $(\eps, \delta)$-DP algorithm \alg is $\left(\ell \eps, \delta' \right)$-DP for groups of size $\ell$, where $\delta' = \delta\frac{e^{\ell \eps} -1}{e^\eps-1}$; that is, for all datasets $\vec{\dstream}, \vec{\dstream}'$ such that $\|\vec{\dstream} - \vec{\dstream}' \|_0 \leq \ell$,
\begin{equation*}
    \alg(\vec{\dstream}) \approx_{\ell \eps, \delta'}   \alg(\vec{\dstream}').
\end{equation*}
\end{lemma}


Differential privacy is closed under post-processing.
\begin{lemma}[Post-Processing~\cite{dwork2006calibrating,BunS16}]\label{prelim:postprocess} If $\alg$  is an $(\eps, \delta)$-DP algorithm with output space $\mathcal{Y}$ and $\mathcal{B}$  is a randomized map from $\mathcal{Y}$ to $\mathcal{Z}$, then the algorithm $\mathcal{B} \circ \alg$ is $(\eps, \delta)$-DP.
\end{lemma}

\begin{definition}[Sensitivity] Let $f: \X^n \rightarrow \R^m$ be a function. Its $\ell_1$-sensitivity is
\begin{equation*}
    \sup_{\text{neighbors } \vec{\dstream}, \vec{\dstream}' \in \X^n} \|f(\vec{\dstream}) - f(\vec{\dstream}')\|_1.
\end{equation*}
To define $\ell_2$-sensitivity, we replace the $\ell_1$ norm with the $\ell_2$ norm.
\end{definition}

We use the standard Laplace and exponential mechanisms to ensure differential privacy. 

\begin{definition}[Laplace Distribution] The Laplace distribution with parameter $b$ and mean $0$, denoted  $\Lap(b)$,
has probability density
\begin{equation*}
    h(r) = \frac{1}{2b}e^{-\frac{|r|}{b}} \text{ for all $r \in \mathbb{R}$}.
\end{equation*}
\end{definition}

\begin{lemma}[Laplace Mechanism, \cite{dwork2006calibrating}]\label{prelim:laplace_dp} Let $f : \X^n \rightarrow \mathbb{R}^m$ be a function with $\ell_1$-sensitivity at most $\Delta_1$. Then the Laplace mechanism is algorithm
\begin{equation*}
    \alg_f(\vec{\dstream}) = f(\vec{\dstream}) + (Z_1, \ldots, Z_m),
\end{equation*}
where $Z_i \sim \Lap\left(\frac{\Delta_1}{\eps}\right)$. Algorithm $\alg_f$ is $(\eps, 0)$-DP.
\end{lemma}

\begin{lemma}[Exponential Mechanism \cite{McTalwar}]\label{lem:expmech}
Let $L$ be a set of outputs and $g: L \times \X^n \to \mathbb{R}$ be a function that measures the quality of each output on a dataset. Assume that for every $m \in L$, the function $g(m,.)$ has $\ell_1$-sensitivity at most $\Delta$. Then, for all $\eps,n > 0$ and  all datasets $\dset \in \X^n$, there exists an $(\eps, 0)$-DP mechanism that outputs an element $m\in L$ such that, for all $a>0$,
\begin{equation*}
    \Pr[\max_{i \in [L]} g(i,\dset) -  g(m,\dset) \geq 2\Delta \frac{(\ln |L| + a)}{\eps}] \leq e^{-a}. 
\end{equation*}
\end{lemma}


%%%%%%%%%%%%%%%%%%% rho zCDP prelims %%%%%%%%%%%%%%%%
\subsection{Facts on $\rho$-zCDP}\label{sec:zCDP}

This section contains facts about {\em zero-concentrated differential privacy} (zCDP). It differs from $(\eps,\delta)$-differential privacy in that zCDP requires output distributions on all pairs of neighboring datasets to be $\rho$-close (\Cref{def:rho-indistinguishable}) instead of $(\eps,\delta)$-indistinguishable.
In \Cref{sec:upper-bounds}, we prove that our mechanisms are zCDP and then use conversion to $(\eps,\delta)$-differential privacy (\Cref{prop:CDPtoDP}) to compare our upper and lower bounds.

\begin{definition}[R\'enyi Divergence \cite{Renyi61}]
Let $Q$ and $Q'$ be distributions on $\mathcal{Y}$. For $\xi \in (1,\infty)$, the R\'enyi divergence of order $\xi$ between $Q$ and $Q'$(also called the $\xi$-R\'enyi Divergence) is defined as
\begin{align}
    D_{\xi}(Q \| Q') = \frac{1}{\xi-1} \log\left( \E_{r \sim Q'} \left[ \left(\frac{Q(r)}{Q'(r)}\right)^{\xi-1} \right]  \right).
\end{align}
Here $Q(\cdot)$ and $Q'(\cdot)$ denote either probability masses (in the discrete case) or probability densities (when they exist). More generally, one can replace  $\frac{Q(.)}{Q'(.)}$ with the the Radon-Nikodym derivative of $Q$ with respect to $Q'$.
\end{definition}

\begin{definition}[$\rho$-Closeness]\label{def:rho-indistinguishable}
Random variables $R_1$ and $R_2$ over the same outcome space $\mathcal{Y}$ are  {\em $\rho$-close} (denoted $R_1 \simeq_{\rho} R_2$) if for all $\xi \in (1,\infty)$, 
\begin{align*}
D_{\xi}(R_1\|R_2) \leq \xi\rho \text{ and }  D_{\xi}(R_2\|R_1) \leq \xi\rho,
\end{align*}
where $D_{\xi}(R_1\|R_2)$ is the $\xi$-R\'enyi divergence  between the distributions of $R_1$ and $R_2$.
\end{definition}


\begin{definition}[zCDP in Batch Model~\cite{BunS16}]
A randomized batch algorithm $\alg : \X^n \to \mathcal{Y}$ is $\rho$-zero-concentrated differentially private ($\rho$-zCDP), if, for all neighboring datasets $\vec{\dset},\vec{\dset}' \in \mathcal{X}^n$,
$$\alg(\vec{\dset}) \simeq_{\rho} \alg(\vec{\dset'}).$$
\end{definition}

One major benefit of using zCDP is that this definition of privacy admits a clean composition result. 
%We use it when analyzing the privacy of the algorithms in \Cref{sec:upper-bounds}.

\begin{lemma}[Composition \cite{BunS16}] \label{lem:cdp_composition}
Let $\alg : \mathcal{X}^n \to \mathcal{Y}$ and $\alg' : \mathcal{X}^n \times \mathcal{Y} \to \mathcal{Z}$ be batch algorithms. Suppose $\alg$ is $\rho$-zCDP and $\alg'$ is $\rho'$-zCDP. Define batch algorithm $\alg'' : \mathcal{X}^n \to \mathcal{Y} \times \mathcal{Z}$ by $\alg''(\vec{\dset}) = \alg'(\yvec,\alg(\yvec))$. Then $\alg''$ is $(\rho+\rho')$-zCDP.
\end{lemma}

The \emph{Gaussian mechanism}, defined next,
%is used in \Cref{sec:upper-bounds}. It 
privately estimates a real-valued function by adding Gaussian noise to its value. %The following lemma shows that the Gaussian mechanism is zCDP.

\begin{definition}[Gaussian Distribution] The Gaussian distribution with parameter $\sigma$ and mean 0, denoted $\Gauss(0,\sigma^2)$, has probability density
\begin{equation*}
    h(r) = \frac{1}{\sigma \sqrt{2\pi}} e^{-\frac{r^2}{2\sigma^2}}  \text{ for all $r \in \mathbb{R}$}.
\end{equation*}
\end{definition}


\begin{lemma}[Gaussian Mechanism \cite{BunS16}] \label{prop:gaussian-mech}
Let $f : \X^n \to \mathbb{R}$ be a function with $\ell_2$-sensitivity at most $\Delta_2$. Let $\alg$ be the batch algorithm 
%$\alg : \mathcal{X}^n \to \mathbb{R}$ 
that, on input $\yvec$, releases a sample from $\mathcal{N}(f(\yvec), \sigma^2)$. Then $\alg$ is $(\Delta_2^2/2\sigma^2)$-zCDP.
\end{lemma}

The final lemma in this section relates zero-concentrated differential privacy to $(\eps,\delta)$-differential privacy.

\begin{lemma}[Conversion from zCDP to DP \cite{BunS16}]\label{prop:CDPtoDP}
For all $\rho,\delta > 0$, if batch algorithm $\alg$ is $\rho$-zCDP, then $\alg$ is $(\rho+2\sqrt{\rho \log(1/\delta)},\delta)$-DP.
\end{lemma}


\subsection{Useful Concentration Inequalities}
\begin{lemma}\label{lem:gauss_conc}
For all random variables $R \sim \gauss(0,\sigma^2)$,
\begin{equation*}
    \Pr[|R| > \ell] \leq 2e^{-\frac{\ell^2}{2 \sigma^2}}.
\end{equation*}
\end{lemma}
\begin{lemma}\label{lem:gauss_max}
Consider $m$ random variables $R_1,\dots,R_m \sim \gauss(0,\sigma^2)$. Then
\begin{equation*}
    \Pr[\max_{j \in [m]} |R_j| > \ell] \leq 2 m e^{-\frac{\ell^2}{2 \sigma^2}}.
\end{equation*}
\end{lemma}
\begin{proof}
By a union bound and Lemma~\ref{lem:gauss_conc},
\begin{align*}
    \Pr[\max_{i \in [m]} |R_i| > \ell] 
      = \Pr( \exists i \in [m] \text{ such that } |R_i| > \ell) \\
     \leq \sum_{i=1}^m \Pr( |R_i| > \ell) \leq
    \sum_{i=1}^m  2e^{-\frac{\ell^2}{2 \sigma^2}}  =  2m e^{-\frac{\ell^2}{2 \sigma^2}}.
\end{align*}
\end{proof}
A similar union bound argument yields the following concentration inequality on the maximum of the absolute values of i.i.d.\ Laplace random variables.
\begin{lemma}\label{lem:lapmax}
Fix $m \in \N$, $\lambda > 0$. Consider $m$ random variables $R_1,\dots,R_m \sim Lap(\lambda)$. Then for all $a>0$,
$$\Pr(\max_{i \in [m]} |R_i| > \lambda (\log m + \log a) ) \leq e^{-a}.$$
\end{lemma} 



\section{Proofs  Omitted from Section~\ref{sec:selection-lowerbound}}\label{app:sec4proofs}

Item~1 in Lemma~\ref{lem:kindsel-mainlb} follows from \Cref{lem:lbkindsel} below.
\begin{theorem}[\cite{US17,Ullman21pers}]\label{lem:lbkindsel}
For all $\epsilon \in (0,1], \delta \in (0,1/n]$, $\gamma \in [0,\frac{1}{20}]$, $d,n,k \in \N$, if Algorithm $\alg$ is $(\eps,\delta)$-differentially private and $(\gamma,n)$-accurate for $\kindselection{d}$, then $n = \Omega(\frac{\sqrt{k}\log d}{\gamma \eps \log (k+1)})$.
\end{theorem}
\begin{proof}[Proof Sketch]
We are aware of two proofs of this result, both of which were communicated to us by Jonathan Ullman~\cite{Ullman21pers}. The first uses the top-$k$ selection lower bound of Steinke and Ullman~\cite{US17}. In that problem, there is a single collection of $d$ coordinates and the goal is to return the indices of $k<d$ coordinates whose sums are roughly largest. 

% \as{The specific  distribution over instances that arises in the lower bound of~\cite{US17} has two useful properties: first, the contents of the dataset's $dk$ coordinates ... IN PRGORESS. }
For the specific distribution over instances that arises in the lower bound of~\cite{US17}, if one divides the coordinates into $k$ equal groups, there is a constant probability that the collection of coordinates with the largest sum in each group is a good approximate solution for the top-$k$ selection problem. An algorithm for $\kindselection{d}$ can thus be used to solve the top-$k$ selection (out of $dk$ coordinates) problem for such instances with roughly the same error and privacy parameter. The lower bound of~\cite{US17} on $n$ then applies.

Another approach is to use the composition framework of Bun, Ullman and Vadhan \cite{bunUV18}. One can use a folklore result that selection among $d>2^m$ coordinates can be used to mount a reconstruction attack on an appropriate dataset of size $m$. Composed with the lower bound for 1-way marginals in \cite{bunUV18}, one obtains a lower bound for $\kindselection{d}$.
\end{proof}
%The following lemma is used to add an appropriate dependence on $\eps$ to \Cref{lem:lbkindsel}. This lemma appears to be folklore. We've added a proof of it in the appendix for completeness.
%\begin{lemma}\label{lem:boost-eps}
%\asnote{I think we can remove this lemma entirely.}Let $n,d,k \in \N$. If every $(1,o(\frac{1}{ndk})$-DP and $(\frac{n}{20},n)$-accurate algorithm for $\kindselection{d}$ in the batch model requires $n > g(k,d)$ records for some function $g$, then for all $\eps \in (0,1]$, every $\left(\eps,o(\frac{1}{ndk})\right)$-DP and $(\frac{n}{20},n)$-accurate algorithm for $\kindselection{d}$ in the batch model requires $n >  \frac{g(k,d)}{\eps}$ records.
%Let $n,d,k \in \N, \epsilon \in (0,1], \delta \in (0,1/ndk]$. Let $\alg$ be and $(\eps,\delta)$-differentially private, $(\frac{kn}{20},n)$-accurate algorithm for $\kindselection{dk}$ then $n = \Omega(\frac{\sqrt{k}\log d}{\eps})$
%\end{lemma}
To complete the proof of \Cref{lem:kindsel-mainlb}, we prove Item $2$ via a standard packing argument. 
%\begin{lemma}\label{thm:purekindselLB}
%Let $n,d,k \in \N, \epsilon \in (0,1]$, $0 < \gamma < \frac{n}{3}$. If $\alg$ is an $(\eps,0)$-differentially private and $(\gamma,n)$-accurate algorithm for $\kindselection{d}$, then $n = \Omega(\frac{k\log d}{\eps})$.
%\end{lemma}
\begin{proof}[Proof of \Cref{lem:kindsel-mainlb},  Item~2.]
For $\vec{u}\in [d]^k,$ let $\dset^*_{\vec{u}} \in \zo^{dk}$ be the record where each block $r\in[k]$ of $d$ coordinates has a $1$ in coordinate $u_r$ and zeros everywhere else. Let $\vec{\dset_u}$ be the dataset that consists of $2\gamma n$ copies of~$\dset^*_{\vec{u}}$ and $(1-2\gamma)n$ copies of the all-zero record (assume, for simplicity, that $2\gamma n$ is an integer). Since $\alg$ is $(\gamma,n)$-accurate,\\
$\Pr_{\text{coins of \alg}}\left[ \err_{\kindselection{}}(\vec{\dset_u},\alg(\vec{\dset_u})) \leq \gamma \right] \geq \frac{2}{3}$ for all $\vec{u}\in[d]^k$. This means that for all $\vec{u}\in[d]^k$,
\[\Pr_{\text{coins of \alg}}\left[\alg(\vec{\dset_u}) = \vec{u}\right] \geq \frac{2}{3}.\]
For all $\vec{u},\vec{u}' \in [d]^k$, by group privacy,
$\alg(\vec{\dset_u}) \approx_{(\gamma\eps n,0)} \alg(\vec{\dset_{u'}})$, which implies that
\begin{align}\label{eq:groupprivlb}
\Pr\left[\alg(\vec{\dset_{u}}) = \vec{u}'\right] &\geq e^{-\gamma\eps n}\Pr\left[\alg(\vec{\dset_{u'}}) = \vec{u}'\right] \geq \frac{2}{3}e^{-\gamma\eps n}.
\end{align}
Since the probability of any event is at most 1,
\begin{align*}
& 1\geq \Pr_{\text{coins of \alg}}\left[ \alg(\vec{\dset_u}) \neq \vec{u} \right] = \\
& \sum_{\vec{u}'\neq \vec{u}}\Pr\left[\alg(\vec{\dset_u}) = \vec{u}'\right] \geq \frac{2}{3}e^{-\gamma\eps n}(d^k-1),
\end{align*}
where the last inequality holds by (\ref{eq:groupprivlb}). We get that
$e^{\gamma\eps n} \geq \frac{d^k-1}{2}\cdot\frac{2}{3}$, and thus $n = \Omega\left(\frac{k\log d}{\gamma \cdot \eps}\right).$
%The probability that $\alg$ outputs the wrong answer on input $\vec{\dset_u}$ is the following, where the last inequality follows by (\ref{eq:groupprivlb}):
%\[
%\Pr_{\text{coins of \alg}}\left[ \err_{\kindselection{}}(\vec{\dset_u},\alg(\vec{\dset_u})) \geq \gamma \right] = %\sum_{u'\neq u}\Pr\left[\alg(\vec{\dset_u}) = u'\right] \geq \frac{2}{3}e^{-\eps n}(d^k-1).
%\]
%Using the fact that any probability is trivially upper bounded by $1$,
%\begin{align*}
%   1 \geq \frac{2}{3}e^{-\eps n}(d^k-1) \implies e^{\eps n} \geq \frac{d^k}{2}\cdot\frac{2}{3} \implies n = %\Omega\left(\frac{k\log d}{\eps}\right).
%\end{align*}
\end{proof}

\section{Details Omitted from Section~\ref{sec:upper-bounds}}\label{sec:details_ub}
\subsection{Formal Statements}\label{sec:adaptive-up-statments}
\fi
%In this section do both the accuracy proofs first and then add the privacy proofs after because the accuracy doesn't need the simulator game
In this subsection, we state theorems that summarize the performance guarantees of our mechanisms for $\maxsum{d}$ and $\selection{d}$. We prove these theorems in the following subsections. The upper bounds in these theorems are attained by two simple mechanisms: one uses the binary tree mechanism and the other recomputes the target function at regular intervals. We first state results for the binary-tree-based approach.

%The idea of recomputing at regular intervals applies quite generally. Item 1 of Theorem \ref{thm:recompute_rho} for general sensitivity-1 functions (which include $\maxsum{d}$); a similar result holds for bounded sensitivity functions with output space $\R^d$. 

%We state guarantees for the algorithm  in terms of sensitivity-1 functions; these apply, in particular, to $\maxsum{d}$. 
% In particular, more broadly to sensitivity-1 functions $f$ with output space $\R$. This result\srnote{This mechanism? It is not clear what is meant by ``result'' here.} can be extended to the case of bounded sensitivity functions with output space $\R^d$.\pjnote{is this description clear?}

%\begin{theorem}\label{thm:sens1_rho}
%For all $\rho \in (0,1]$, sufficiently large $T > 0$, and all functions $f:\X^* \to \R$ such that $\Delta_f \leq 1$, there exists a mechanism $\mech$ for $f$ that is $\rho$-zCDP and $(\alpha,T)$-accurate in the \aCR{}, where $\alpha = \BigO{\min\{T,\frac{T^{1/3} \sqrt{\log T}}{\rho^{1/3}}\}}$.
%\end{theorem}
%Additionally, we prove the following upper bound for the $\maxsum{d}$
%problem (which has $\ell_1$-sensitivity $1$).
%\begin{theorem}\label{thm:maxsum_rho}
%For all $\rho \in (0,1]$, $d \in \N$ and sufficiently large $T > 0$, %there exists a mechanism $\mech$ for $\maxsum{d}$ that is $\rho$-zCDP %and $(\alpha,T)$-accurate in the \aCR{}, where $\alpha = %\BigO{\frac{\sqrt{d} \log T \sqrt{\log(Td)}}{\sqrt{\rho}}}$.
%\end{theorem}
%For $\selection{d}$, we prove the following upper bounds.
%\begin{theorem}\label{thm:sel_rho1}
%For all $\rho \in (0,1]$, $d \in \N$, and sufficiently large $T > 0$, there exists a mechanism $\mech$ for $\selection{d}$ that is $\rho$-zCDP and $(\alpha,T)$-accurate in the \aCR{}, where $\alpha = \BigO{\frac{\sqrt{d} \log T \sqrt{\log(Td)}}{\sqrt{\rho}}}$.
%\end{theorem}
%\begin{theorem}\label{thm:sel_rho2}
%For all $\rho \in (0,1]$, $d \in \N$, and sufficiently large $T > 0$, there exists a mechanism $\mech$ for $\selection{d}$ that is $\rho$-zCDP and $(\alpha,T)$-accurate in the \aCR{}, where $\alpha = \BigO{\min\left\{T, \frac{T^{1/3} (\log T  + \log d)}{\rho^{1/3}} \right\} }$.
%\end{theorem}

\begin{theorem}[zCDP, Binary-Tree-Based Mechanisms]\label{thm:bintree_rho}
For all $\rho \in (0,1]$, $d \in \N$, and sufficiently large $T > 0$, there exist $\rho$-zCDP mechanisms $\mech, \mech'$ in the \aCR{} such that $\mech$ is $(\alpha,T)$-accurate for $\maxsum{d}$ and $\mech'$ is $(\alpha,T)$-accurate for $\selection{d}$, where $\alpha = \BigO{\frac{\sqrt{d} \log T \sqrt{\log(dT)}}{\sqrt{\rho}}}$.
\end{theorem}

The next theorem uses the idea of recomputing at regular intervals, which applies quite generally. Item 1 of Theorem~\ref{thm:recompute_rho} applies for general sensitivity-1 functions (which include $\maxsum{d}$); a similar result holds for bounded-sensitivity functions with output space $\R^d$. 

\begin{theorem}[zCDP, Mechanisms via Recomputing at Regular Intervals]\label{thm:recompute_rho}
For all $\rho \in (0,1]$, $d \in \N$, sufficiently large $T > 0$, and all functions $f:\X^* \to \R$ with $\ell_2$-sensitivity at most $1$, there exist $\rho$-zCDP mechanisms $\mech$ and $\mech'$ in the \aCR{} such that

\begin{enumerate}
    \item Mechanism $\mech$ is $(\alpha,T)$-accurate for $f$ for \ifnum \pods=1 \\ \fi $\alpha \allowbreak = \BigO{\min\left\{ \sqrt[3]{\frac{T\log T}{\rho}},T \right\}};$
    \item Mechanism $\mech'$ is $(\alpha,T)$-accurate for $\selection{d}$ for $\alpha = \BigO{\min\left\{ \frac{T^{1/3}\log^{2/3}(d T)  }{\rho^{1/3}}, T \right\} }$.
\end{enumerate} 
\end{theorem}


Combining Theorems~\ref{thm:bintree_rho}--\ref{thm:recompute_rho}, using the conversion from zCDP to $(\eps, \delta)$-DP from \Cref{prop:CDPtoDP} and substituting $\rho = \frac{\eps^2}{16 \log(1/\delta)}$, we get the following corollary.
\begin{corollary}\label{cor:upper-bounds}
For all $\eps \in (0,1]$, $\delta \in (0,\frac{1}{2}]$, $d \in \N$, and sufficiently large $T > 0$, there exist $(\eps, \delta)$-DP mechanisms $\mech$ and $\mech'$ in the \aCR{} such that\\
(1) $\mech$ is $(\alpha,T)$-accurate for $\maxsum{d}$ for 
\ifnum\pods=1
\\
\else
\fi
$\alpha = \BigO{\min\left\{ \frac{\sqrt[3]{T\log(1/\delta)\log T} }{\eps^{2/3}}, \frac{\sqrt{d\log(dT) \log(1/\delta)}\,\log T}{\eps}, T \right\}};$\\
(2) $\mech'$ is $(\alpha,T)$-accurate for $\selection{d}$ for
\ifnum\pods=1
\\
\else
\fi
$\alpha = \BigO{ \min \left\{\frac{\sqrt[3]{T \log^2 (dT) \log(1/\delta)}  }{\eps^{2/3}},  \frac{ \sqrt{d\log(dT) \log(1/\delta)} \, \log T}{\eps} , T \right\}}$. 
\end{corollary}

Simple variants of our mechanisms can be used to get the following theorems for $(\eps,0)$-differential privacy. 

\begin{theorem}[Pure DP, Binary-Tree-Based Mechanisms]\label{thm:bintree_pure}
For all $\eps \in (0,1]$, $d \in \N$, and sufficiently large $T > 0$, there exist $(\eps,0)$-DP mechanisms $\mech$ and $\mech'$ in the \aCR{} such that $\mech$ is $(\alpha,T)$-accurate for $\maxsum{d}$ and $\mech'$ is $(\alpha,T)$-accurate for $\selection{d}$ for $\alpha = \BigO{\frac{d (\log d) \log^3 T}{\eps}}$.
\end{theorem}

\begin{theorem}[Pure DP, Mechanisms via Recomputing at Regular Intervals]\label{thm:recompute_pure}
For all $\eps \in (0,1]$, $d \in \N$, sufficiently large $T > 0$, and all functions $f:\X^* \to \R$ with $\ell_1$-sensitivity at most $1$, there exist $(\eps,0)$-DP mechanisms $\mech$ and $\mech'$ in the \aCR{} such that
\begin{enumerate}
    \item Mechanism $\mech$ is $(\alpha,T)$-accurate for $f$ for
\ifnum\pods=1
\\
\else
\fi
    $\alpha = \BigO{\min\left\{\sqrt{\frac{T\log T}{\eps}},\,T \ \right\}};$
    \item Mechanism $\mech'$ is $(\alpha,T)$-accurate for $\selection{d}$ for 
\ifnum\pods=1
\\
\else
\fi
$\alpha = \BigO{\min\left\{\sqrt{\frac{T \log (dT)  }{\eps}},\,T \right\} }.$
\end{enumerate}
\end{theorem}
Theorems~\ref{thm:bintree_pure}--\ref{thm:recompute_pure} yield the following corollary.

\begin{corollary}\label{cor:pure_dp}
For all $\eps \in (0,1]$, $d \in \N$, and sufficiently large $T > 0$, there exist $(\eps, 0)$-DP mechanisms $\mech$ and $\mech'$ in the \aCR{} such that
\begin{enumerate}
    \item  $\mech$ is $(\alpha,T)$-accurate for $\maxsum{d}$ for
\ifnum\pods=1
\\
\else
\fi
$\alpha = \BigO{\min\left\{\sqrt{\frac{T\log T}{\eps}},\,T, \frac{d (\log d) \log^3 T}{\eps} \ \right\}};$\\
    \item Mechanism $\mech'$ is $(\alpha,T)$-accurate for $\selection{d}$ for $\alpha = \BigO{\min\left\{\sqrt{\frac{T \log (dT)  }{\eps}},\,T,\frac{d (\log d) \log^3 T}{\eps} \right\} }$.
\end{enumerate}
\end{corollary}



%The following notation is used multiple times in following subsections. We define $[i:j]$ for natural numbers $i \leq j$ to be all the natural numbers $\{i, \dots, j\}$.  
%%%%%%%%%%%%%%%%%%%%%%%% SELECTION UPPER BOUNDS %%%%%%%%%%%%%%
\subsection{Algorithms based on the Binary Tree Mechanism}

In this section, we prove \Cref{thm:bintree_rho} for $\selection{d}$. \Cref{thm:bintree_rho} for $\maxsum{d}$ follows from the same analysis by considering the binary tree mechanism that outputs the highest noisy sum instead of the coordinate that achieves it.

In order to approximate $\selection{d}$ on a dataset with $d$ attributes, we use the binary tree mechanism from \cite{ChanSS10,DworkNPR10} to privately sum each of the attributes of the records $\xt$ received so far, and then choose the attribute with the highest sum. For simplicity of exposition, in this section, we assume that $T$ is a power of 2. In general, we can work with the smallest power of 2 greater than $T$. Throughout this section, $[i:j]$, where $i,j\in \mathbb{N}$, denotes the set of natural numbers $\{i, \dots, j\}$.


%%%%%%%%%%%%%%%%%%%%%%%%%%%% ALGORITHM %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\nleft}{\ell}
\newcommand{\nright}{r}

\ifnum\pods=0
\begin{algorithm}[h!]
\else
\begin{algorithm*}[h!]
\fi
    \caption{Mechanism $\mech$ for $\selection{d}$ in \aCR{}}
    \label{alg:selbintree}
    \hspace*{\algorithmicindent}
    \begin{algorithmic}[1]
           \Statex\textbf{Input:} time horizon $T \in \N$, privacy parameter $\rho$, stream $\vec{\dstream} = (\dstream_1,\dots,\dstream_T) \in \X^T$, where $\X = \{0,1\}^d$.
           \Statex\textbf{Output:} stream $(a_1,\dots,a_T) \in [d]^T$.
           \State\textbf{Initialization:} Construct a complete binary tree with $T$ leaves labeled $\node_{[1:1]},\dots,\node_{[T:T]}$. Label every internal node  $\node_{[\nleft:\nright]}$
            %where  $\node_{[\nleft,\nleft]}$ is the label of the leftmost leaf in $\node_{[\nleft,\nright]}$'s subtree, and $\node_{[\nright,\nright]}$ is the label of the rightmost leaf in $\node_{[\nleft,\nright]}$'s subtree. 
            if the subtree rooted at that node has leaves  $\node_{[\nleft:\nleft]},\dots,\node_{[\nright:\nright]}.$
            Initialize the partial sum $\nodeval_{[\nleft:\nright]}\gets 0^d$ for each node $\node_{[\nleft:\nright]}$ in the tree.
            \For{\text{$t=1$ to $T$}}
               \State Get record $\dstream_t$ from $\adv$. 
               
               \emph{$\triangleright$ Compute noisy sums for nodes completed at time $t$}
               \For{\text{each node $\node_{[\nleft:t]}$}}
               \State Draw noise $Z \sim \gauss(0,\sigma^2 \mathbb{I}^{d \times d})$, where $\sigma = \sqrt{\frac{d(\log T+1)}{2\rho}}$, and set $\nodeval_{[\nleft:t]} \gets \sum_{i=\nleft}^{\nright} \dstream_i +Z.$
               \label{line:noisebintree}
               %\State $\nodeval_{[\nleft:t]} \gets \sum_{i=\nleft}^{\nright} \dstream_i +Z.$
               \EndFor
               
               \emph{$\triangleright$ Output Steps:}
               
               \ifnum\pods=0
               \State  \label{step:output-start} $I_t \gets $ 
               \parbox[t]{5.5in}{collection  of at most $\log t + 1$ disjoint intervals whose union is $[1:t]$ and where  each interval labels a node in the binary tree. (See Remark~\ref{rem:bintree_dyadic}.)}
               \else
               \State  \label{step:output-start} $I_t \gets $ 
               \parbox[t]{5.5in}{collection  of at most $\log t + 1$ intervals that partition $[1:t]$, where  each interval labels a node in the binary tree. (See Remark~\ref{rem:bintree_dyadic}.)}
               \fi
               \State $\mathsf{sum}_t \gets \sum_{[\nleft:\nright] \in I_t}  \nodeval_{[\nleft:\nright]}$. \label{step:noisysumvec}
               \State  Output $a_t \gets \argmax_{j \in [d]} \mathsf{sum}_t[j]$. \label{step:a_tchoice} \label{line:outputselect}
               \EndFor
    \end{algorithmic}
\ifnum\pods=1
\end{algorithm*}
\else
\end{algorithm}
\fi
%Here is a compact description (adapted from~\cite{SmithT13}) of 
At the high level, the binary tree mechanism constructs a complete binary tree with $T$ leaves. The leaves correspond to the input records 
%$\dstream_1,\dots,\dstream_T$, 
$\xt$, where each record $\dstream_i\in\zo^d$. Each internal node in the tree corresponds to the sum of all the leaves in its subtree. 
%In a differentially private version of this tree, we ensure that each node's subtree 
Each node stores the noisy version of the corresponding sum 
computed by adding a noise vector drawn from $\gauss(0,\sigma^2 \mathbb{I}^{d \times d})$ with $\sigma = \sqrt{\frac{d (\log T+1)}{2\rho}}.$ The algorithm that releases the noisy sum is $\frac{\rho}{\log T+1}$-zCDP.
Since each $\dstream_t$ participates in only $\log_2 T +1$ sums in the tree, by \emph{adaptive composition} of zCDP (\Cref{lem:cdp_composition}), the complete mechanism is $\rho$-zCDP (\Cref{thm:bintree_rho}). The sum of all the attributes at any timestep can be calculated by adding at most $\log T$ of the sums stored in the tree, one at each level. The algorithm that adds the corresponding noisy sums is $(\alpha,T)$-accurate for $\alpha\approx\BigO{ \frac{\sqrt{d} \log T \log(Td)}{\sqrt{\rho}}}$. The formal description of the algorithm appears in \Cref{alg:selbintree}. The algorithm uses a dyadic decomposition (described in Remark~\ref{rem:bintree_dyadic}) to decide which nodes of the tree it accesses to compute any particular output.

%%%%%%%%%%%%%%%%%%%%%%%%%%%% PRIVACY %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}[H]
%    \centering
%    \includegraphics[width=0.95\textwidth]{images/Untitled.png}
%    \caption{This picture needs editing}
%    \label{fig:binary_sim}
%\end{figure}
\begin{remark}[Dyadic Decomposition]\label{rem:bintree_dyadic}
For any natural number $t>1$, the interval $[1:t]$ can be expressed as a union of at most $\log t + 1$ disjoint intervals as follows. Consider the binary expansion of $t$ (which has at most $\log t + 1$ bits), and express $t$ as a sum of distinct powers of $2$ ordered from higher to lower powers. Then, the first interval $[1:r]$ will have size equal to the largest power of $2$ in the sum. The second interval will start at $r+1$ and its size will be equal to the second largest power of $2$ in the sum. Similarly, the remaining intervals are defined until all terms in the summation have been exhausted. For example, for $t=7=4+2+1$, the intervals are $[1:4]$, $[5:6]$ and $\{7\}$.
\end{remark}

We  present the privacy and accuracy analysis for \Cref{alg:selbintree} in Lemmas~\ref{lem:privbintree} and~\ref{lem:accbintree}, respectively, which together prove \Cref{thm:bintree_rho} for $\selection{}$. 



\begin{lemma}\label{lem:privbintree}
For all $\rho \in \R^{+}$, $d,T \in \N$, mechanism $\mech$ described in \Cref{alg:selbintree} is $\rho$-zCDP in the \aCR.
\end{lemma}

\ifnum\pods=1
\begin{algorithm*}[h!]
\else
\begin{algorithm}[h!]
\fi
    \caption{Simulator $\Sim$ for the proof of \Cref{lem:privbintree}}
    \label{alg:binary_sim}
    \begin{algorithmic}[1]%\onehalfspacing
        \Statex \textbf{Input:} \Longunderstack[l]{time horizon $T \in \N$, privacy parameter $\rho\in\R^{+}$, black-box access to an adversary $\adv$ and \\ a mechanism $\idealgauss$.}
        \Statex \textbf{Output:} stream $(a_1,\dots,a_T) \in [d]^T$.
        \Statex \textbf{$\boldsymbol{\adv}$:} \Longunderstack[l]{
         At each timestep $t\in[T]\setminus\{t^*\}$, $\adv$ provides $\Sim$ with record $\dstream_t\in\X$, where $\X = \{0,1\}^d$.
         At \\the challenge timestep~$t^*$ (chosen by $\adv$), it provides records $\dstream_{t^*}^{(L)}, \dstream_{t^*}^{(R)} \in \X$. 
         At each timestep\\ $t\in[T]$, $\Sim$ provides $\adv$ with output $a_t\in [d]$.}
        \Statex \textbf{$\boldsymbol{\idealgauss}$:} $\Sim$ exchanges $\log_2 T + 1$ messages with $\idealgauss$.
        \State \textbf{Initialization:} Perform Step~1 (the initialization phase) of \Cref{alg:selbintree}.
        \State $j \gets 1$.
        \For{\text{$t\in [T]$}}
            \If{\text{$t = t^*$}}
                \State Get input $(\dstream_{t^*}^{(L)}, \dstream_{t^*}^{(R)})$ from $\adv$.
                \For{\text{$i \in [\log T + 1]$}}
                    \State Send $(\dstream_{t^*}^{(L)}, \dstream_{t^*}^{(R)})$ to $\idealgauss$, and get back a response $p_i$.
                \EndFor
            \Else
                \State Get record $\dstream_t$ from $\adv$.
            \EndIf
            \For{\text{each node $\node_{[\nleft,t]}$}}
                \If{$t^* \not\in [\nleft:t]$ where $[\nleft:t]$ denotes the integers $\{\nleft, ..., t\}$}
                    \State Draw noise $Z \sim \gauss(0,\sigma^2 \mathbb{I}^{d \times d})$, where $\sigma = \sqrt{\frac{d (\log T+1)}{2\rho}}$.
                    \State $\nodeval_{[\nleft:t]} \gets Z + \sum_{i=\nleft}^{\nright} \dstream_i$
                \Else\label{algline:contains_challenge_bintree}
                    \State $\node_{[\nleft:t]} \gets \sum_{i \in [\nleft:t]\setminus\{t^*\}} \dstream_i + p_j$. 
                    \State $j \gets j+1$.
                \EndIf
            \EndFor
            \State \Longunderstack[l]{\emph{Output Steps:}} Perform Steps~\ref{step:output-start}--\ref{step:a_tchoice} (the output steps) of \Cref{alg:selbintree}.
        \EndFor
    \end{algorithmic}
\ifnum\pods=0
\end{algorithm}
\else
\end{algorithm*}
\fi


\begin{algorithm}[h!]
\caption{Mechanism $\idealgauss$}
\label{alg:ideal_gauss}
    \begin{algorithmic}[1]
        \Statex \textbf{Input:} $\side \in \{L, R\}$ (not known to $\Sim$).
        \Statex \textbf{Output:} A natural number.
        \For{\text{$i=1$ to $\log T + 1$}}
            \State Get records $\node_i^{(L)}$, $\node_i^{(R)} \in \zo^d$ from $\Sim$.
            \State Draw noise from a multivariate Gaussian distribution $Z \sim \gauss(0,\sigma^2 \mathbb{I}^{d \times d})$, where $\sigma = \sqrt{\frac{d(\log T+1)}{2\rho}}$.\label{algline:idealgauss-sigma}
            \State Output $\node_i^{(\side)} + Z$
        \EndFor
%        \State  Return $V_{\mech,\adv}^{(side)}$
    \end{algorithmic}
\end{algorithm}

\begin{proof}
Consider an adversary $\adv$ interacting with the privacy game $\Pi_{\mech,\adv}$. We want to argue that the adversary's view is $\rho$-close in the two versions of the privacy game (for the two possible values of $\side \in \{L,R\}$.)  We will achieve this by introducing a $\rho$-zCDP mechanism $\idealgauss$ with input $\side$ and reducing our goal to the privacy of $\idealgauss$. 

For this, we use a simulation argument similar to those used in cryptography. Specifically, our proof defines two algorithms: (a) a $\rho$-zCDP mechanism $\idealgauss$ that gets input $\side \in \{L,R\}$ and (b) a simulator $\Sim$ with query access to $\idealgauss$ that does not know the value of $\side$. The simulator $\Sim$ interacts with adversary $\adv$ and satisfies a key guarantee: 
\begin{quote}
    The view of the adversary $\adv$ in its interaction with $\Sim$ is identically distributed to its view in the privacy game $\Pi_{\mech,\adv}$, defined in \Cref{alg:privacy_game}.   (\Cref{fig:sim_diagram} illustrates the structure of these two kinds of interaction.)
\end{quote} 

Since the simulator's outputs to $\adv$ are a post-processing of the query responses from $\idealgauss$, we can argue that the adversary's view is $\rho$-close in the two versions of the privacy game $\Pi_{\mech,\adv}$.


\begin{figure*}
    \centering
    \ifnum\pods=1
    \includegraphics[width={0.9\textwidth}]{images/sim_diagram.png}
    \else 
    \includegraphics[scale =0.35]{images/sim_diagram.png}
    \fi
    \caption{An illustration of the simulation argument from the proof of \Cref{lem:privbintree}. The left-hand side shows the game used to define privacy with adaptively selected inputs. The right-hand side shows the simulation structure described in the proof. For each value of $\side$, the adversary's view is identical in these two settings.}
    \label{fig:sim_diagram}
\end{figure*}

%To show that the view of the adversary $\adv$ in its interaction with $\Sim$ is identically distributed to its view in the privacy game $\Pi_{\mech,\adv}$, we want the probability that $\adv$ can guess the value of $\side$ in the privacy game to be the same as the probability that $\adv$ can guess the value of $\side$ in its interaction with $\Sim$. Then, since the simulator doesn't know the value of $\side$, $\adv$ can only learn as much about $\side$ from its interaction with $\Sim$ as one can learn by querying $\idealgauss$. Intuitively then, if $\idealgauss$ does not reveal much about the value of $\side$ then neither does $\mech$.

To see why this is helpful, recall that we want to show that the probability of $\adv$ guessing the value of $\side$ in the privacy game is small. If the probability of $\adv$ guessing the value of $\side$ is the same in the privacy game as in its interaction with $\Sim$, then—since the simulator doesn't know the value of $\side$—$\adv$ can only learn as much about $\side$ from its interaction with $\Sim$ as one can learn by querying $\idealgauss$. Intuitively, if $\idealgauss$ does not reveal much about the value of $\side$ then neither does $\mech$. We now describe $\idealgauss$ and the simulator, and formalize the argument.

The mechanism $\idealgauss$ (described in \Cref{alg:ideal_gauss}) gets  an input $\side \in \{L,R\}$. It receives at most $\log T + 1$ queries of the form $v^{(L)},v^{(R)}$ from $\Sim$ to which it responds with $p = v^{(\side)} + Z$ where the noise $Z$ is drawn from $\gauss(0,\sigma^2 \mathbb{I}^{d \times d})$ for $\sigma = \sqrt{\frac{d (\log T+1)}{2 \rho}}$. Observe that if $\idealgauss$ has only a single interaction with $\Sim$ and outputs a single noised value, then by the privacy guarantee of the Gaussian mechanism (Lemma~\ref{prop:gaussian-mech}), $\idealgauss$ is $\frac{\rho}{\log T+1}$-zCDP. This can be seen by imagining that $\idealgauss$ is computing a function $f(\side) = \dstream_i^{\side}$ and observing that the $\ell_2$-sensitivity of $f$ is $\sqrt{d}$. Since there are $\log T +1$ interactions between $\idealgauss$ and $\Sim$, $\idealgauss$ is an adaptive composition of $\log T+1$ algorithms, each of which is $\frac{\rho}{\log T+1}$-zCDP. By \Cref{lem:cdp_composition} on composition, $\idealgauss$ is $\rho$-zCDP. 

The simulator $\Sim$ (described in \Cref{alg:binary_sim}) interacts with the adversary without knowing the input $\side \in \{L,R\}$ that is given to $\idealgauss$. It queries $\idealgauss$ exactly $\log T + 1$ times and uses the query responses to provide outputs to the adversary. The aim of the simulator is to mimic the behaviour of $\Pi_{\mech,\adv}$ even though it doesn't know $\side$. The simulator constructs a binary tree as described in \Cref{alg:selbintree}. 
For all nodes in the binary tree except for those whose interval contains the challenge timestep $t^*$, 
the computation of the noisy subtree sums 
can be done by $\Sim$ without any help from $\idealgauss$. For the nodes whose interval does contain $t^*$, the simulator sends $(x_{t^*}^{(L)},x_{t^*}^{(R)})$ to $\idealgauss$ and gets a noisy value of $x_{t^*}^{\side}$. It can then compute the corresponding subtree sum by adding the input records corresponding to the remaining leaves. Notice that the simulator can produce these outputs  online---at the same time that $\Pi_{\mech,\adv}$ would.

The crucial point to note is that the view of the adversary $\adv$ in the privacy game $\Pi_{\mech,\adv}$ is identically distributed to its view in the interaction with $\idealgauss$ and $\Sim$. Furthermore, the view of the adversary $\adv$ when interacting with $\Sim$ and $\idealgauss$ is simply a post-processing of the outputs provided to it by $\Sim$, which are a post-processing of the outputs provided to $\Sim$ by $\idealgauss$. Hence,
$$\idealgauss\text{ is }\rho\text{-zCDP } \implies V_{\mech,\adv}^{(L)}\simeq_{\rho} V_{\mech,\adv}^{(R)}.$$

It remains to argue that exactly $\log T+1$ nodes have a subtree sum that depends on the inputs from the challenge timestep $t^*$. Each node $\node_{[\nleft,\nright]}$ whose subtree sum depends on the inputs from timestep $t^*$ satisfies $t^*\in [\nleft:\nright]$. This holds only for one node at each level of the binary tree created by $\Sim$ (because the intervals represented by the nodes at a particular level are disjoint.) Since the binary tree has depth $\log T + 1$, exactly $\log T+1$ nodes have a subtree sum that depends on the inputs from the challenge timestep $t^*$. 
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% ACCURACY %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}\label{lem:accbintree}
For all $\rho > 0$ and sufficiently large $T \in \N$, mechanism $\mech$ is $(\alpha,T)$-accurate for $\selection{}$ in the \aCR{}  for $\alpha = \BigO{ \frac{\sqrt{d} \log T \sqrt{\log(Td)}}{\sqrt{\rho}}}$.
\end{lemma}
\begin{proof}
Consider any adversarial process $\adv$ interacting with $\mech$.
%
We  first argue that, at every timestep~$t$, the random variable $ \err_{\selection{d}}(\xt, a_t)$ corresponding to the error at any timestep~$t$ can be upper bounded by a random variable that is the sum of at most $2\log t$ independent Gaussian random variables. We then use tail bounds for Gaussian random variables, along with a union bound, to argue that, with high probability, the maximum value of this random variable is not too large. Finally, we take a union bound over timesteps to argue that, with high probability, $\max_{t\in [T]} \err_{\selection{d}}(\xt, a_t)$ is not too large.

First, at any timestep~$t$, let $sum_t$ represent the vector of noisy sums defined in Step~\ref{step:noisysumvec} of \Cref{alg:selbintree}. Therefore, each coordinate of this sum, $sum_t[j] = \sum_{i\in [t]} \dstream_t[j] + \sum_{i\in [|I_t|]} Z_i$ is the sum of at most $\log t+1$ noisy interval sums. Here, $Z_i$ is a Gaussian random variable with mean $0$ and standard deviation $\sigma = \sqrt{\frac{d(\log T+1)}{2\rho}}$, and all $Z_i$s are mutually independent. Hence, by the linearity of expectation, and by the linearity of the variance of independent random variables, we get that $\sum_{i\in [|I_t|]} Z_i$ is a Gaussian random variable with mean $0$ and standard deviation $\sqrt{\frac{d(\log T+1)|I_t|}{2\rho}} \leq \sqrt{\frac{d(\log T+1)(\log t + 1)}{2\rho}}$. Consider the vector $N$ consisting of the absolute values of $d$ random variables independently drawn from the distribution $\gauss(0,\sigma^2)$ where $\sigma = \sqrt{\frac{d|I_t|(\log T+1)}{2\rho}}$. The distribution of $N$ is identical to the component-wise absolute values of the Gaussian noise vector $sum_t - \sum_{i\in [t]} \dstream_i$. Then,
$$\sum_{i\in [t]} \dstream_i[a_t] + \max_{j \in [d]} N[j] \geq \maxsum{d}(\xt) - \max_{j \in [d]} N[j],$$ 
since if $a_t$ is selected at timestep~$t$, the noisy sum of coordinate $a_t$ at timestep~$t$ is larger than the noisy sums of all other coordinates at timestep~$t$ (see Step~\ref{step:a_tchoice} in \Cref{alg:selbintree}). Thus,
\ifnum\pods=0
$$\err_{\selection{d}}(\xt, a_t) = \maxsum{d}(\xt) - \sum_{i\in [t]} \dstream_i[a_t] \leq 2 \max_{j \in [d]} N[j].$$
\else
\begin{align*}
&\err_{\selection{d}}(\xt, a_t)\\ = &\quad \maxsum{d}(\xt) - \sum_{i\in [t]} \dstream_i[a_t] \leq 2 \max_{j \in [d]} N[j].
\end{align*}
\fi
Next, we reason about $\max_{j \in [d]} N[j]$ using standard probability tools. Set $\ell = \sqrt{10\frac{d(\log T+1)(\log t+1) \log(dT)}{2\rho}}.$ By Lemma~\ref{lem:gauss_max} on concentration of the maximum of the absolute values of Gaussian random variables, and since
$\sigma \leq \sqrt{\frac{d(\log T+1)(\log t + 1)}{2\rho}}$, we get that
$$\Pr [\max_{j \in [d]} N[j] > \ell] \leq 2d e^{-\frac{\ell^2}{2\sigma^2}} \leq 2d e^{-5\log(dT)} \leq \frac{2}{T^{5}}.$$ 
Then,  with probability at most $\frac{2}{T^{5}}$ (over the coins of the algorithm $\alg$ and the adversarial process $\adv$), 
\begin{align*}
\err(\xt, a_t) &> 20 \sqrt{\frac{d(\log T+1)(\log t+1) \log(dT)}{2\rho}}\\
&\geq 20 \sqrt{\frac{d(\log T+1)^2\log(dT)}{2\rho}},
\end{align*}
since $t \leq T$.
By a union bound over all $t \in [T]$, we get that $\max_{t\in [T]} \err_{\selection{d}}(\xt, a_t) > 20 \sqrt{\frac{d(\log T+1)^2 \log(dT)}{2\rho}}$ 
with probability at most $\frac{2}{T^{4}} \leq \frac{1}{3}$ for sufficiently large~$T$. 
This proves the lemma.
\end{proof}
\begin{proof}[Proof Sketch of Theorem~\ref{thm:bintree_pure}]
The proof of Theorem~\ref{thm:bintree_pure} for $\selection{d}$ closely follows the exposition above. The mechanism used is the same as Algorithm~\ref{alg:selbintree}, except that in Line~\ref{line:noisebintree}, $Z$ is drawn from $Lap(\frac{d(\log T + 1)}{\eps})$ instead of a Gaussian distribution. The privacy proof is exactly as in Lemma~\ref{lem:privbintree}, except that we use that the composition of $\log T + 1$ mechanisms that are $\big(\frac{\eps}{\log T + 1},0\big)$-DP is $(\eps, 0)$-DP instead a composition theorem for $\rho$-zCDP. The accuracy proof closely follows that of Lemma~\ref{lem:accbintree}, with the main difference being that the the vector $N$ is defined as the component-wise absolute value of $d$ random variables independently drawn from the distribution of the sum of $|I_t|$ independent random variables distributed as $Lap\left(\frac{d(\log(T)+1)}{\eps}\right)$. We  then use the concentration inequality for the maximum of the absolute values of independent Laplace random variables over $d|I_t|$ random variables in Lemma~\ref{lem:lapmax} with $a = 2 \log T$ to argue that the absolute value of each Laplace random variable is smaller than 
$\frac{d(\log T + 1)}{\eps}(\log(d|I_t|) + 10 \log T)$ with probability at least $\frac{1}{T^{10}}$. This implies that $\max_{j \in [d]} N[j]$ is smaller than 
$\frac{d(\log T + 1)^2}{\eps}(\log(d(\log T+1)) + 10 \log T)$ with probability at least $\frac{1}{T^{10}}$, upper bounding $|I_t|$ by $\log T + 1$. Taking a union bound over $T$ and using the fact that $\log(d(\log T + 1)) \leq \log d (\log T + 1)$ for sufficiently large $T$ completes the proof.
\end{proof}
Theorems~\ref{thm:bintree_rho} and~\ref{thm:bintree_pure} for $\maxsum{d}$ are proved analogously. The main difference is that we output $\max_{j \in [d]} sum_t[j]$ instead of $\argmax_{j \in [d]} sum_t[j]$ in \Cref{line:outputselect} of \Cref{alg:selbintree}.

%%%%%%%%%% Sensitivity one functions %%%%%%%%%%%%%%%%%%
\subsection{Algorithms that Recompute at Regular Intervals}\label{sec:maxsum-upperbounds}

In this section, we prove Item~1 of \Cref{thm:recompute_rho} for sensitivity-1 functions. The proof of Item~2 of \Cref{thm:recompute_rho} builds on  the same idea of recomputing $\selection{d}$ every $T/m$ timesteps, but it uses the report noisy max (with exponential noise) algorithm for $\selection{d}$ \cite{McSheldon} instead of adding Gaussian noise to the function. We omit the details, since the argument is essentially the same as in the rest of this section.

The mechanism recomputes the function every $r$ timesteps. Between recomputations, it outputs the most recently computed value. We select $r$ to balance the privacy cost of composition with the error due to returning stale values between recomputations.

\begin{algorithm}[H]
    \caption{Mechanism $\mech$ for sensitivity-$1$ functions in \aCR}
    \label{alg:maxsum}
    \hspace*{\algorithmicindent}
    \begin{algorithmic}[1] % The number tells where the line numbering should start
        \Statex\textbf{Input:} time horizon $T$, privacy parameter $\rho > 0$, recompute period $r \in [T-1]$, function $f$, stream $\vec{\dstream} = (\dstream_1,\dots,\dstream_T) \in \X^n$ where $\X = \{0,1\}^d$.  \Statex\textbf{Output:} stream $(a_1,\dots,a_T) \in \R^T$.
        \State $m \gets \lfloor\frac{T-1}{r}\rfloor$.
        \For{\text{$k=1$ to $m$}}
        \State Get input record $\dstream_{(k-1)r+1}$. 
        \State Draw $Z_k \sim \gauss(0,\sigma^2)$, where $\sigma = \sqrt{\frac{m}{2\rho}}$.   
               \label{line:gaussnoiserecom}
               \State Output $a_{(k-1)r+1} \gets f(\vec{\dstream}_{[(k-1)r+1]} ) + Z_k$. \label{line:noise_sensone}
               \For{\text{$t=(k-1)r+2$ to $kr$}}
                  \State Get input record $\dstream_t$.
                  \State Output $a_t \gets a_{(k-1)r+1}$. \label{line:recompute_sensone}
               \EndFor
             \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{claim}\label{lem:privmax}
For all $\rho, T > 0$, $r \in [T-1]$, mechanism $\mech$ defined in \Cref{alg:maxsum} is $\rho$-zCDP in the \aCR{}.  
\end{claim}

%%%%%%%%%%%%%%%%%%%%% PRIVACY PROOF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{proof}
Consider an adversary $\adv$ interacting with $\mech$. We define a mechanism \sstext{$\idealrecomp$}, similar to \Cref{alg:ideal_gauss}, and a simulator $\Sim$ that interacts with the adversary $\adv$ such that the view of adversary $\adv$ in the interaction with $\idealrecomp$ and $\Sim$ is identically distributed to its view in the privacy game $\Pi_{\mech,\adv}$, defined in \Cref{alg:privacy_game}. 

\begin{algorithm}[h!]
\caption{Mechanism $\idealrecomp$}
\label{alg:ideal_recomp}
    
    \begin{algorithmic}[1]
        %\Statex Let $f$ be a known function with L2 sensitivity $\Delta_f = 1$. 
        \Statex \textbf{Input:} $\side \in \{L, R\}$ (not known to $\Sim$) %, function $f$ with L2 sensitivity $\Delta_f = 1$.
        \Statex \textbf{Output:} A natural number.
        \State Get neighboring datasets $\vec{\dset}^{(L)}$, $\vec{\dset}^{(R)} \in \zo^d$ and a function $f$ with $\ell_2$ sensitivity  at most $1$ from $\Sim$.
        \State Draw noise $Z \sim \gauss(0,\sigma^2)$, where $\sigma = \sqrt{\frac{m}{2\rho}}$.
        \State Output $f\left(\dset^{(\side)}\right) + Z$
%        \State  Return $V_{\mech,\adv}^{(side)}$
    \end{algorithmic}
\end{algorithm}


\ifnum\pods = 1
\begin{algorithm*}[h!]
\else
\begin{algorithm}[h!]
\fi
    \caption{Simulator $\Sim$ for the proof of \Cref{lem:privmax}}
    \label{alg:recompute_sim}
    \begin{algorithmic}[1]%\onehalfspacing
        \Statex \textbf{Input:} time horizon $T$, privacy parameter $\rho > 0$, recompute period $r \in [T-1]$, function $f$. $\Sim$ also has black-box access to an adversary $\adv$ and a process $\idealrecomp$.
        \Statex \textbf{Output:} stream $(a_1,\dots,a_T) \in \R^T$
        \Statex \textbf{$\boldsymbol{\adv}$:} \Longunderstack[l]{
         At each timestep $t\in[T]\setminus\{t^*\}$, $\adv$ provides $\Sim$ with record $\dstream_t\in\X$. At the challenge timestep~$t^*$\\ (chosen by $\adv$), it provides two records $\dstream_{t^*}^{(L)}, \dstream_{t^*}^{(R)}\in\X$. At every timestep $t\in[T]$, $\Sim$ provides \\$\adv$ with output $a_t\in \R$.}
        \Statex \textbf{$\boldsymbol{\idealrecomp}$:} $\Sim$ exchanges $T/r$ messages with $\idealrecomp$.
        \State \textbf{Initialization:} $m \gets \as{\lceil\frac{T}{r}\rceil} $, $j \gets 1$.
        \State For timesteps $t<t^*$, run mechanism $\mech$ in \Cref{alg:maxsum} with inputs from $\adv$, with the same $T, \rho, r, f$. Let $a_t$ be $\mech$'s output at timestep $t$.
        \For{\text{$t \geq t^*$}}
            \If{\text{$t = t^*$}}
                \State Get input $(\dstream_{t^*}^{(L)}, \dstream_{t^*}^{(R)})$ from $\adv$. 
                %\For{\sstext{\sout{\text{$i \in [m]$}}}}
                %    \State \sstext{\sout{Send $(\dstream_{t^*}^{(L)}, \dstream_{t^*}^{(R)})$ to $\idealgauss$, and get back a response $p_i$}}.
                %\EndFor
            \EndIf
            \If{\text{$t \neq t^*$}}
                \State Get record $\dstream_t$ from $\adv$.
            \EndIf
            \If{$t \mod r = 1$}
                %\State \sstext{Let $f_t$ be the function defined by $f_t(\dstream) = f\left(\dstream_{[t^*-1]},\dstream,\dstream_{t^*+1},\dots, \dstream_{t})\right)$}. 
                \State Let $\vec{\dset}^{(\side)}_t = \{\dstream_1,\dots,\dstream_{t^*-1},\dstream^{(\side)}_{t^*},\dstream_{t^*+1},\dots,\dstream_t\}$ \as{for each $\side \in \{L,R\}$}
                \State \sstext{ 
                $a_t \gets \idealrecomp\left(f, \vec{\dset}_t^{(L)}, \vec{\dset}_t^{(R)}\right)$.}
            \Else
                \State $q \gets \lfloor \frac{t}{r}\rfloor$; output $a_t \gets a_{q +1}$. 
            \EndIf
            \EndFor
    \end{algorithmic}
\ifnum\pods = 0
\end{algorithm}
\else
\end{algorithm*}
\fi
%\sstext{I think the next 2 paragraphs should be replaced by the red text below.}
%The mechanism $\idealgauss$ is exactly as described in \Cref{alg:ideal_gauss}, except that in Step~\ref{algline:idealgauss-sigma} it sets $\sigma = \sqrt{\frac{dm}{2\rho}}$. Similarly to the proof of \Cref{lem:privbintree}, each of the $m$ interactions between $\idealgauss$ and $\Sim$ are $\frac{\rho}{m}$-zCDP. We can reason about the overall privacy of $\idealgauss$ by thinking about it as an adaptive composition of $m$ algorithms, each of which are $\frac{\rho}{m}$-zCDP, and correspond to a single interaction with $\Sim$. Applying \Cref{lem:cdp_composition} on composition then gives us that $\idealgauss$ is $\rho$-zCDP.

%Since the function it accepts has $\ell_2$ sensitivity $1$, each of the $m$ interactions between $\idealgauss$ and $\Sim$ are $\frac{\rho}{m}$-zCDP. We can reason about the overall privacy of $\idealgauss$ by thinking about it as an adaptive composition of $m$ algorithms, each of which are $\frac{\rho}{m}$-zCDP, and correspond to a single interaction with $\Sim$. Applying \Cref{lem:cdp_composition} on composition then gives us that $\idealgauss$ is $\rho$-zCDP.

\sstext{The mechanism $\idealrecomp$ is defined in Algorithm~\ref{alg:ideal_recomp}. Since the function $f$ has $\ell_2$ sensitivity at most $1$, then by the privacy of the Gaussian mechanism, and since the variance of the noise added is $\frac{m}{2\rho}$), $\idealrecomp$ is $\frac{\rho}{m}$-zCDP with respect to the dataset consisting of $\side \in \{L,R\}$.} 
%every timestep $t$ after the challenge timestep at which a recomputation happens, the simulator passes the function with all data except that of the challenge timestep hardcoded to $\idealrecomp$ as well as the pair . B, every interaction between $\idealrecomp$ and $\Sim$ is $\frac{\rho}{m}$-zCDP with respect to the dataset consisting of only the element $\side$. Hence, by adaptive composition, since $\idealrecomp$ is called at most $m$ times by $\Sim$, we get that the output transcript of $\idealrecomp$ is $\rho$-zCDP with respect to the dataset containing $\side$.}

The simulator $\Sim$ (described in \Cref{alg:recompute_sim}) gets inputs from $\adv$, but it does not know the input $\side \in \{L,R\}$ that is given to \sstext{$\idealrecomp$}. It interacts with \sstext{$\idealrecomp$} to provide outputs to the adversary $\adv$. The aim of the Simulator is to mimic the behaviour of $\Pi_{\mech,\adv}$ even though it doesn't know $\side$. For all timesteps $t<t^*$ before the challenge timestep, the simulator behaves exactly like $\mech$. 
%
% \sstext{\sout{Starting at the challenge timestep, for every $t\in[t^*:T]$ where $\mech$ would recompute the noised value of the sum, $\Sim$ queries $\idealgauss$ on $(x_{t^*}^{(L)},x_{t^*}^{(R)})$ and gets a response $p_j$, it then computes \\$f\left((\dstream_1,\dots,\dstream_{t^*-1},p_j,\dstream_{t^*+1},\dots, \dstream_{t-1})\right)$.} }
%
\sstext{Starting at the challenge timestep, for every $t\in[t^*:T]$ where $\mech$ would recompute the noised value of the sum, $\Sim$ sends $\idealrecomp$ the function $f$ as well as neighboring datasets  $\vec{\dset}_t^{(L)}, \vec{\dset}_t^{(R)}$ defined by
$$\vec{\dset}^{(\side)}_t = \{\dstream_1,\dots,\dstream_{t^*-1},\dstream^{(\side)}_{t^*},\dstream_{t^*+1},\dots,\dstream_t\}.$$
Since $\Sim$ queries $\idealrecomp$ at most $m$ times, by adaptive composition, the output transcript of $\idealrecomp$ is $\rho$-zCDP with respect to the dataset consisting of $\side$.}

The view of the adversary $\adv$ in the real privacy game $\Pi_{\mech,\adv}$ is identically distributed to its view in the interaction with \sstext{$\idealrecomp$} and $\Sim$. Furthermore, the view of the adversary $\adv$ when interacting with $\Sim$ and \sstext{$\idealrecomp$} is simply a post-processing of the outputs provided to it by $\Sim$, which are a post-processing of the outputs provided to $\Sim$ by \sstext{$\idealrecomp$}. 
\sstext{As argued previously, the output  of $\idealrecomp$} when $\side = L$ is $\rho$-close to its output \sstext{transcript} when $\side  = R$. Hence we have that $V_{\mech,\adv}^{(L)}\simeq_{\rho} V_{\mech,\adv}^{(R)}$.
\end{proof}

\begin{claim}\label{lem:acc-max-delta}
Fix $\rho > 0$, sufficiently large $T > 0$, and $2 \leq m \leq T$. Let $f:\X^* \to \Z$ be a function with $\ell_2$-sensitivity at most $1$. Then mechanism $\mech$, defined in \Cref{alg:maxsum} is $(\alpha, T)$-accurate for $f$ in the \aCR{} where $\alpha = \frac{T}{m} + \sqrt{\frac{10m \log m}{\rho}}.$
\end{claim}

\begin{proof}
Consider any adversarial process $\adv$ interacting with $\mech$. Fix a timestep~$t \in [T]$. Consider time horizon $T$ divided into $m$ stages, where the stage $k\in[m]$ is from timestep $(k-1)r+ 1$ to $kr$. Let timestep~$t$ be in  stage $k$. Intuitively, since $\mech$, defined in \Cref{alg:maxsum}, corresponds to recomputing the noisy sum every $r$ timesteps (and using each recomputed value for the next $r$ timesteps), the error can be decomposed into two parts: one caused by the drift in the true value of the function since the last recomputation and the other caused by noise addition. By the triangle inequality,
\ifnum\pods=0
\begin{align*}
    \err_f(\xt, a_t) 
    &= \abs{a_t - f(\xt)} \\
    &\leq \abs{f(\xt) - f(\vec{\dstream}_{[(k-1)r+1}]}) + \abs{a_t - f(\vec{\dstream}_{[(k-1)r+1}]}) \\
    & \leq T/m + \abs{a_{(k-1)r+1} - f(\vec{\dstream}_{[(k-1)r+1]})} 
    \leq \frac{T}{m} + \abs{Z_k}.
\end{align*}
\else
\begin{align*}
    & \err_f(\xt, a_t) 
    = \abs{a_t - f(\xt)} \\
    &\leq \abs{f(\xt) - f(\vec{\dstream}_{[(k-1)r+1}]}) + \abs{a_t - f(\vec{\dstream}_{[(k-1)r+1}]}) \\
    & \leq T/m + \abs{a_{(k-1)r+1} - f(\vec{\dstream}_{[(k-1)r+1]})} 
    \leq \frac{T}{m} + \abs{Z_k}.
\end{align*}
\fi
The second inequality above holds because the $\ell_2$-sensitivity of $f$ is at most $1$, and since we recompute every $r=T/m$ timesteps, the maximum change in the function $f$ since the last recomputation is $T/m$. The third inequality follows from Steps~\ref{line:noise_sensone} and~\ref{line:recompute_sensone} in \Cref{alg:maxsum}. Finally, observe that $Z_k$ for $k \in [m]$ are mutually independent Gaussian random variables with mean $0$ and standard deviation $\sqrt{\frac{m}{2\rho}}$. Hence, applying Lemma~\ref{lem:gauss_max} on the concentration of the maximum of the absolute values of Gaussian random variables (setting $\ell = \sqrt{\frac{10 m \log m}{\rho}}$), and using the fact that $m \geq 2$, 
\ifnum\pods=0
\begin{align*}
    \Pr_{\text{coins of }\alg,\adv}\left( \max_{t\in[T]} \err_f(\xt,a_t) \geq \frac{T}{m} + \sqrt{ \frac{10m \log m}{\rho}} \right) & =
    \Pr_{\text{coins of }\alg,\adv}\left( \max_{k\in[m]} |Z_k| \geq \sqrt{ \frac{10m \log m}{\rho}} \right) \\
    & \leq \frac{2}{m^9} \leq \frac{1}{3}.\qedhere
\end{align*}
\else
\begin{align*}
    & \Pr_{\text{coins of }\alg,\adv}\left( \max_{t\in[T]} \err_f(\xt,a_t) \geq \frac{T}{m} + \sqrt{ \frac{10m \log m}{\rho}} \right) \\ =
    & \Pr_{\text{coins of }\alg,\adv}\left( \max_{k\in[m]} |Z_k| \geq \sqrt{ \frac{10m \log m}{\rho}} \right) \leq \frac{2}{m^9} \leq \frac{1}{3}. \qedhere
\end{align*}
\fi
\end{proof}
%We are now ready to prove Item~1 of \Cref{thm:recompute_rho}.
\begin{proof}[Proof of Item~1 in \Cref{thm:recompute_rho}]
By Claim~\ref{lem:privmax}, the mechanism $\mech$ is $\rho$-zCDP in the \aCR{}. 

For $\rho \leq \frac{\log T}{T^2}$, consider the mechanism that doesn't touch the data and always outputs $0$. Clearly it is $0$-zCDP. Additionally, for this mechanism, $\alpha = O(T)$. For $\rho > \frac{\log T}{T^2}$, by Claim~\ref{lem:acc-max-delta}, mechanism $\mech$ is $(\alpha, T)$-accurate for $f$ in the \aCR{}, where $\alpha = T/m + 10\sqrt{\frac{m \log m}{\rho}}$. Setting $m = \lfloor \frac{\rho^{1/3} T^{2/3}}{\log^{1/3} T} \rfloor$ gives $\alpha = \BigO{\min \left\{T, \sqrt[3]{\frac{T \log T}{\rho}} \right\}}$, where the $\min$ comes from the option of using the trivial mechanism. 
\end{proof}

\begin{proof}[Proof Sketch of Item~1 in \Cref{thm:recompute_pure}]
The mechanism $\mech$ used is a variant of \Cref{alg:maxsum}. The only difference is that in Line~\ref{line:gaussnoiserecom}, instead of the random variable $Z_k$ being distributed as a Gaussian, it is distributed as $Lap(\frac{m}{\eps})$. The privacy proof follows a structure similar to that of Claim~\ref{lem:privmax}, with the main difference being that instead of using a composition theorem for $\rho$-zCDP, we instead use that the composition of $m$ mechanisms that are $(\frac{\eps}{m},0)$-DP is $(\eps, 0)$-DP. 

For accuracy, we can prove a claim phrased exactly as  Claim~\ref{lem:acc-max-delta}, with $\alpha = \frac{T}{m} + \frac{m}{\eps}[ \log m + 2 \log T ]$ instead of $\alpha = \frac{T}{m} + \sqrt{\frac{10m \log m}{\rho}}$. The proof is similar, with the only difference being that instead of using Lemma~\ref{lem:gauss_max} on the maximum of i.i.d. Gaussian random variables, we instead use Lemma~\ref{lem:lapmax} on the maximum of i.i.d. Laplace random variables, with $t = 2\log T$.

Finally, we prove the theorem as follows: for $\eps > \frac{\log T}{T}$, setting $m = \lfloor \sqrt{\frac{\eps T}{\log T}} \rfloor$ in the accuracy claim gives $\alpha = O(\sqrt{\frac{T}{\eps}\log T})$. For $\eps \leq \frac{\log T}{T}$, we can consider the mechanism that always outputs $0$ at every timestep. This mechanism is $(0,0)$-DP and $(\alpha, T)$-accurate for $f$ in the \aCR{} with $\alpha = O(T)$. This completes the proof.
\end{proof}
\begin{proof}[Proof Sketch of Item~2 in Theorems~\ref{thm:recompute_rho} and \ref{thm:recompute_pure}]
We \ifnum\pods=1 \\ \fi  sketch the proof of Item 2 of \Cref{thm:recompute_rho}. The proof of Item 2 of \Cref{thm:recompute_pure} is essentially the same. The upper bound mechanism $\mech$ used for this proof is a variant of \Cref{alg:maxsum} where we recompute $\selection{d}$ using the exponential mechanism \cite{McTalwar} with $\eps' = \sqrt{\frac{2\rho}{m}}$ (for Item 2 of \Cref{thm:recompute_pure} on pure DP, we use $\eps' = \frac{\eps}{m}$). The quality function of an attribute and dataset pair is defined to be the sum of that attribute over all entries in the dataset. The exponential mechanism instantiated as described above is used to privately compute $\selection{d}$ every $T/m$ timesteps. Between recomputations, the attribute index produced at the last recomputation is used as the output. 

The privacy proof follows a structure similar to that of Claim~\ref{lem:privmax}. The main difference for this proof is that the simulator will now interact with an ideal mechanism that takes as input a differentially private algorithm as well as neighboring datasets to run the algorithm on. In particular, the neighboring datasets will be the inputs $x_{t^*}^{(L)}$ and $x_{t^*}^{(R)}$ from the challenge timestep, and the algorithm will be the exponential mechanism hardcoded with all the inputs of the adversary so far (except for the inputs from the challenge timestep.) The ideal mechanism will run the algorithm with challenge input $x_{t^*}^{(\side)}$ and output the result. The adversary's view in the privacy game is clearly identical to its view when interacting with the simulator. Finally, the closeness of the adversary's view in the simulated world when $\side = L$ and when $\side = R$ follows directly from the privacy of the exponential mechanism and adaptive composition~\cite{DworkRV10,BunS16}.

For accuracy, we prove a claim akin to  Claim~\ref{lem:acc-max-delta}, with $\alpha = \frac{T}{m} + 2\sqrt{\frac{m}{2\rho}}[ \log d + 5 \log m ]$. The proof is similar to that of Claim~\ref{lem:acc-max-delta}; here, we define $|Z_k|$ as the error incurred by the $k^{th}$ instantiation of the exponential mechanism, and use Lemma~\ref{lem:expmech} on the accuracy of the exponential mechanism (setting $a = 5 \log m$) and take a union bound over the $m$ recomputations to argue that the maximum error is greater than $\alpha = \frac{T}{m} + 2\sqrt{\frac{m}{2\rho}}[ \log d + 5 \log m ]$ with probability at most $\frac{1}{m^4}$.

For $\rho > (\frac{\log (d T)}{T})^2$, by the accuracy claim, mechanism $\mech$ is $(\alpha, T)$-accurate for $f$ in the \aCR{}, where $\alpha = \frac{T}{m} + 2\sqrt{\frac{m}{2\rho}}[ \log d + 2 \log m ]$. Setting $m = \lfloor \frac{\rho^{1/3} T^{2/3}}{(\log (d T)^{2/3}} \rfloor$  yields $\alpha = O\left(\frac{T^{1/3}\log (d T)^{2/3} }{\rho^{1/3}} \right)$. Finally, for $\rho \leq (\frac{\log (d T)}{T})^2$, consider the mechanism that doesn't touch the data and always outputs $0$. It is clearly $0$-zCDP, and has $\alpha = O(T)$.
\end{proof}


%Finally, we convert from $\rho$-zCDP to $(\eps, \delta)$-DP.
%\begin{corollary}\label{thm:sens1_cdp_delta}
%For all $\eps, \delta \in (0,1/2]$, sufficiently large $T>0$ and functions $f:\X^* \to \Z$ such that $\Delta_f > 0$, mechanism $\mech$ defined in \Cref{alg:maxsum} is $(\epsilon, \delta)$-DP and $(\alpha,T)$-accurate in the \aCR{} where $\alpha = \BigO{\min\left\{T,\frac{T^{1/3} \sqrt{\log T} \sqrt[3]{\log 1/\delta}}{\eps^{2/3}}\right\}}.$
%\end{corollary}

%\begin{proof}
%Setting $\rho = \frac{\epsilon^2}{16 \log(1/\delta)}$, we get by \Cref{prop:CDPtoDP} on converting from $\rho$-zCDP to $(\eps, \delta)$-DP and \Cref{lem:privmax} on $\rho$-zCDP of $\mech$, that mechanism $\mech$ is $(\epsilon, \delta)$-DP. 

%Substituting this into the expression for $\alpha$ in Item~\pjnote{?} from \Cref{thm:recompute_rho} proves the corollary.
%\end{proof}
%\begin{theorem}
%For all $d,t \in \N$, the $\ell_1$-sensitivity of the function $\maxsum{d}:\X^t \to \R$ is $1$.  
%\end{theorem}\pjnote{say something about this meaning that our upper bound is tight}

\ifnum\pods=0
\section*{Acknowledgments}

We are grateful to Kobbi Nissim for being part of the conversations that got this work started and for subsequent helpful comments. We are also grateful to Jon Ullman for insights into  the difficulty of the top-$k$ selection problem. 
\else 
\fi


